Hierarchical Adaptive Loco-manipulation Control for Quadruped Robots

Legged robots have shown remarkable advantages in navigating uneven terrain. However, realizing effective locomotion and manipulation tasks on quadruped robots is still challenging. In addition, object and terrain parameters are generally unknown to the robot in these problems. Therefore, this paper proposes a hierarchical adaptive control framework that enables legged robots to perform loco-manipulation tasks without any given assumption on the object's mass, the friction coefficient, or the slope of the terrain. In our approach, we first present an adaptive manipulation control to regulate the contact force to manipulate an unknown object on unknown terrain. We then introduce a unified model predictive control (MPC) for loco-manipulation that takes into account the manipulation force in our robot dynamics. The proposed MPC framework thus can effectively regulate the interaction force between the robot and the object while keeping the robot balance. Experimental validation of our proposed approach is successfully conducted on a Unitree A1 robot, allowing it to manipulate an unknown time-varying load up to $7$ $kg$ ($60\%$ of the robot's weight). Moreover, our framework enables fast adaptation to unknown slopes (up to $20^\circ$) or different surfaces with different friction coefficients.

==> Sections/Background.tex <==
\section{Background} \label{sec:Background}

\subsection{Simplified Robot Dynamic}
\label{sec:simplified robot dynamic}
Due to the complexity of the legged robot, a simplified rigid-body model has been used to present the system's dynamic. This model enables us to calculate the ground reaction forces (GRFs) in real-time. A few  assumptions have been made to achieve simplified robot dynamics\cite{DiCarlo2018DynamicControl}:

\textit{Assumption 1:} The robot has low inertia legs, so their effect is negligible.

\textit{Assumption 2:} For small values of roll ($\phi$) and pitch ($\theta$), the rotation matrix $\bm{R}$ which transforms from the body to world coordinates, can be approximated as the rotation matrix corresponding to the yaw angle ($\psi$):
\begin{align}\label{eq:rotation matrix}
\bm{R} \cong \bm{R}_z(\psi) = \left[\begin{array}{ccc}  
\cos(\psi) & -\sin(\psi) & 0 \\  
\sin(\psi) & \cos(\psi) & 0  \\
0         &      0     & 1
\end{array} \right] 
\end{align}
Therefore, the roll, pitch, and yaw rate of change can be approximated as:
\begin{align}\label{eq:rpy rate of change}
\left[\begin{array}{c}  
\dot{\phi}\\  
\dot{\theta}\\
\dot{\psi}
\end{array} \right] \cong \bm{R}_z(\psi) \bm{\omega}
\end{align}

\textit{Assumption 3:} For small angular velocity, the following approximation can be made: 
\begin{align}
\frac{d}{dt}(\bm{I}_G \bom_b) = \bm{I}_G \dot \bom_b + \bom_b \times (\bm{I}_G \bom_b) \approx \bm{I}_G \dot \bom_b
\end{align}
where $\bm{I}_G\in \mathbb{R}^{3 \times 3}$ is the moment of inertia in the world frame.

Based on the above assumptions, the state representation of the robot dynamic is as follows:
\begin{align}\label{eq:SS}
&\left[\begin{array}{c}  
    \dot{\pos}_{c} \\ 
    \bm{\dot{\Theta}} \\ 
    \ddot{\pos}_{c} \\  
    \dot \bom_{b} 
\end{array} \right] = 
\left[\begin{array}{cccc} 
    \bm{0}_3 & \bm{0}_3 & \bm{I}_3 & \bm{0}_3 \\ 
    \bm{0}_3 & \bm{0}_3 & \bm{0}_3 & \bm{R}_z(\psi)\\ 
    \bm{0}_3 & \bm{0}_3 & \bm{0}_3 & \bm{0}_3 \\ 
    \bm{0}_3 & \bm{0}_3 & \bm{0}_3 & \bm{0}_3
\end{array} \right] 
\left[\begin{array}{c}  
    {\pos}_{c} \\ 
    \bm{\Theta} \\ 
    \dot{\pos}_{c} \\ 
    \bom_{b} 
\end{array} \right] +  \nonumber \\ &
 \left[\begin{array}{ccc} 
\bm{0}_{3} & \dots & \bm{0}_{3} \\
\bm{0}_{3} & \dots & \bm{0}_{3} \\
  \mathbf{I}_{3} / m & \dots & \mathbf{I}_{3}/m \\
    \hspace{-0.1cm}  \bm{I}_G^{-1} [\bm{p}_{1} - \pos_{c}] \times & \dots & \bm{I}_G^{-1} [\bm{p}_{4} - \pos_{c}] \times
  \end{array} \right] \bm{F} + 
\left[\begin{array}{c}
    \bm{0} \\
    \bm{0} \\
    \bm{g} \\
    \bm{0} 
\end{array} \right]
\end{align}
where $m$ is the robot's mass, $\bm{g}\in \mathbb{R}^{3}$ is the gravity vector, $\bm{p}_{c}\in \mathbb{R}^{3}$ is the position of the center of mass (COM), and $\bm{p}_{i}\in \mathbb{R}^{3}$ ($i \in \{1,2,3,4\}$) are the positions of the feet, $\ddot{\pos}_{c}\in \mathbb{R}^{3}$ is body’s linear acceleration, $\dot \bom_b\in \mathbb{R}^{3}$ is angular acceleration, and $\bm{F} = [\bm{F}_1^T, \bm{F}_2^T, \bm{F}_3^T, \bm{F}_4^T]^T \in \mathbb{R}^{12}$ are the ground reaction forces acting on each of the robot’s four feet.

To have the dynamic equation in the convenient state-space form, gravity should be added to the state. So, the system can represent as follows:

\begin{align}\label{eq:convenient SS}
 \bm{\dot{X}} = \bm{D} \bm{X} + \bm{H} \bm{F}   
\end{align}
where 
\begin{align}\label{eq:convenient SS components}
&\bm{X} = \left[\begin{array}{c} 
    \pos_{c} \\ 
    \bm{\Theta} \\ 
    \dot{\pos}_{c} \\ 
    \bom_{b}\\
    ||\bm{g}||
    \end{array} \right] \in \mathbb{R}^{13}
\\ \nonumber
&\bm{D} = \left[\begin{array}{ccccc} 
    \bm{0}_3 & \bm{0}_3 & \bm{I}_3 & \bm{0}_3 & \bm{0}_{3 \times 1}\\ 
    \bm{0}_3 & \bm{0}_3 & \bm{0}_3 & \bm{R}_z(\psi) & \bm{0}_{3 \times 1}\\ 
    \bm{0}_3 & \bm{0}_3 & \bm{0}_3 & \bm{0}_3 & \frac{\bm{g}}{||\bm{g}||}\\ 
    \bm{0}_3 & \bm{0}_3 & \bm{0}_3 & \bm{0}_3 & \bm{0}_{3 \times 1}\\
    \bm{0}_{1 \times 3} & \bm{0}_{1 \times 3} & \bm{0}_{1 \times 3} & \bm{0}_{1 \times 3} & 0
\end{array} \right] \in \mathbb{R}^{13 \times 13} \\ \nonumber
&\bm{H} = \left[\begin{array}{ccc} 
\bm{0}_{3} & \dots & \bm{0}_{3} \\
\bm{0}_{3} & \dots & \bm{0}_{3} \\
  \mathbf{I}_{3} / m & \dots & \mathbf{I}_{3}/m \\
    \hspace{-0.1cm}  \bm{I}_G^{-1} [\bm{p}_{1} - \pos_{c}] \times & \dots & \bm{I}_G^{-1} [\bm{p}_{4} - \pos_{c}] \times \\
    \bm{0}_{1 \times 3} & \dots & \bm{0}_{1 \times 3}
  \end{array} \right] \in \mathbb{R}^{13 \times 12}
\end{align}

\subsection{Model Predictive Control for Locomotion}
\label{sec:mpc}

Model predictive control (MPC) finds the optimal sequence of inputs over the finite-time horizons by considering constraints in the dynamic model. 
We consider a linear MPC problem with horizon length $k$ as follows:
\begin{align}
\label{eq:mpc}
\min_{\bm{F}} \quad & \sum_{i=0}^{k-1} {\bm{e}_{i+1}}^T \bm{Q}_i {\bm{e}_{i+1}} + {\bm{F}_{i}}^T \bm{R}_i \bm{F}_{i} \\ \nonumber
\textrm{s.t.} \quad & \bm{e}_{i+1} = \bm{X}_{i+1} - \bm{X}_{i+1,d} \\ \nonumber
& \bm{X}_{i+1} = \bm{D}_{t,i} \bm{X}_{i} + \bm{H}_{t,i} \bm{F}_{i} \\ \nonumber
& \underline{\bm{\mathfrak{d}}}_i \leq \bm{\mathfrak{C}}_{i} \bm{F}_{i} \leq \bar{\bm{\mathfrak{d}}}_i
\end{align}
where $\bm{X}_{i}$ is the system state at time step $i$, $\bm{X}_{i,d}$ is the system desired state, $\bm{F}_{i}$ is the computed ground reaction forces at time step $i$, $\bm{Q}_i$ and $\bm{R}_i$ are diagonal positive semi-definite matrices, $\bm{D}_{t,i}$ and $\bm{H}_{t,i}$ are discrete time system dynamics matrices.  
The constraint $\underline{\bm{\mathfrak{d}}}_i \leq \bm{\mathfrak{C}}_{i} \bm{F}_i \leq \bar{\bm{\mathfrak{d}}}_i$ represents as\cite{Focchi2017High-slopeRobots}:
\begin{align}
& \bm{\mathfrak{C}}_{i} = \left[\begin{array}{ccc} \bm{C}_1 & \dots & \bm{0}_{5 \times 3} \\ \vdots & \ddots & \vdots \\ \bm{0}_{5 \times 3} & \dots & \bm{C}_4 \end{array}\right]\in \mathbb{R}^{20 \times 12},  \nonumber \\
&\underline{\bm{\mathfrak{d}}}_i = \left[\begin{array}{c} \underline{\bm{d}}_1 \\ \vdots \\  \underline{\bm{d}}_4 \end{array}\right] \in \mathbb{R}^{20}, \quad
\bar{\bm{\mathfrak{d}}}_i = \left[\begin{array}{c} \bar{\bm{d}}_1 \\ \vdots \\  \bar{\bm{d}}_4 \end{array}\right] \in \mathbb{R}^{20}
\end{align}
with
\begin{align}\label{friction}
&\bm{C}_j = \left[\begin{array}{c} (\mu_j \bm{n}_j - {\bm{t}_1}_j)^T \\ (\mu_j \bm{n}_j - {\bm{t}_2}_j)^T \\ (\mu_j \bm{n}_j + {\bm{t}_2}_j)^T \\ (\mu_j \bm{n}_j + {\bm{t}_1}_j)^T \\ {\bm{n}_j}^T \end{array}\right]\in \mathbb{R}^{5 \times 3},  \nonumber \\
&\underline{\bm{d}}_j = \left[\begin{array}{c} 0 \\ 0 \\  0 \\ 0 \\ {f_{min}}_j \end{array}\right] \in \mathbb{R}^{5}, \quad
\bar{\bm{d}}_j = \left[\begin{array}{c} \infty \\ \infty \\  \infty \\ \infty \\ {f_{max}}_j \end{array}\right] \in \mathbb{R}^{5}
\end{align} 
where $\mu_i$ is the coefficient of friction, $\bm{n}_i \in \mathbb{R}^{3}$ is the direction normal to the surface, ${\bm{t}_1}_i, {\bm{t}_2}_i \in \mathbb{R}^{3}$ are the tangential directions, ${f_{max}}_i$, ${f_{min}}_i$ are the upper and lower bound for the $i$th normal force, respectively. This constraint ensures that the optimized forces lie inside the friction pyramid and the normal forces stay within a feasible range.

\subsection{Desired Trajectory}
The desired trajectory is generated based on the robot's velocity command. The robot operator commands $xy$-velocity and yaw rate, then $xy$-position and yaw are determined by integrating the corresponding velocity. $z$ position contains a constant value of $0.3 m$, and the remaining states (roll, roll rate, pitch, pitch rate, and $z$-velocity) are always zero.

\subsection{Swing Leg Control}



==> Utils/TestCommands.tex <==
% File used to test the custom commands for various equations and variables used in the paper.

% Titles the section 
\section{Test Commands}

State Variable Definitions\\
$\roll \pitch \yaw \dRoll \dPitch \dYaw \omegaX \omegaY \omegaZ\\
\quatVector \posVector \angVelVector \velVector \rpyVector \rpyDotVector\\
\stateVector \stateVectorRed \inputVector\\
\rpyVector = \quatToRPY\\
\rpyDotVector = \omegaToRPYDot\angVelVector$\\\\

Simplified Dynamics\\
$\inputForceTorqueFunction = \inputForceTorque = \forceTorqueTransform\uToForceTorqueMat\BMat{\forceEstimate_1 \\ \vdots \\ \forceEstimate_s}\\
\simpleDynamics$\\\\

Direct Collocation Decision Variables\\
$\decisionArrayVector\\
\decisionArrayVectorFull$\\\\

Model Predictive Control Formulation\\
$\basicCostFunction\\
\basicCost = \MPCCostFull\\
\stateError = \stateErrorFull\\
\inputError = \inputErrorFull\\
\basicCostFunction = \MPCCostFunction$\\

% MPC Formulation (descriptive titles)
\begin{equation*}
	\begin{matrix}
		&\MPCMin
		&   & \MPCSum\pMat{\MPCCost}_{n,k} \\\\
		& \text{subject to}
		&	& \text{Dynamics} \\
		  &   &   & \dynamicsConstraint                \\\\
		  &   &   & \text{Foot placed on ground}       \\
		  &   &   & \groundConstraint                  \\\\
		  &   &   & \text{Kinematic leg limits}        \\
		  &   &   & \kinematicLegConstraint            \\\\
		  &   &   & \text{Foot stationary in stance}   \\
		  &   &   & \slipConstraint                    \\\\
		  &   &   & \text{Lateral force friction cone} \\
		  &   &   & \frictionConstraint{x}             \\
		  &   &   & \frictionConstraint{y}             
	\end{matrix}
\end{equation*}

% MPC Formulation (just equations)
\begin{equation*}
	\begin{matrix}
		&\MPCMin
		&   & \MPCSum\pMat{\MPCCost}_{n,k} \\\\
		& \text{subject to}
		&   & \dynamicsConstraint     \\
		  &   &   & \groundConstraint       \\
		  &   &   & \kinematicLegConstraint \\
		  &   &   & \slipConstraint         \\
		  &   &   & \frictionConstraint{x}  \\
		  &   &   & \frictionConstraint{y}  \\
	\end{matrix}
\end{equation*}
